AutoML in Heavily Constrained Applications

Optimizing a machine learning pipeline for a task at hand requires careful configuration of various hyperparameters, typically supported by an AutoML system that optimizes the hyperparameters for the given training dataset. Yet, depending on the AutoML system's own second-order meta-configuration, the performance of the AutoML process can vary significantly. Current AutoML systems cannot automatically adapt their own configuration to a specific use case. Further, they cannot compile user-defined application constraints on the effectiveness and efficiency of the pipeline and its generation. In this paper, we propose CAML, which uses meta-learning to automatically adapt its own AutoML parameters, such as the search strategy, the validation strategy, and the search space, for a task at hand. The dynamic AutoML strategy of CAML takes user-defined constraints into account and obtains constraint-satisfying pipelines with high predictive performance.

==> 07_acknowledge.tex <==
\begin{acks}
This work was funded by the German Ministry for Education and Research as BIFOLD - Berlin Institute for the Foundations of Learning and Data (ref. 01IS18025A and ref. 01IS18037A).
\end{acks}

==> 0_revision.tex <==
\twocolumn 
[\begin{center}
    \mbox{\LARGE\bf Response to Reviewer Comments}
    % {\LARGE\bf Response Letter for ``\system: Effective Error Correction \newline via a Unified Context Representation and Transfer Learning''}
\end{center} 
\vspace*{1em}
]

Dear Reviewers, \\


thank you for your constructive feedback and the chance to improve our paper in this revision. In this letter, we respond to each of your comments in detail. To quickly identify how we address each reviewer's points, we color code the answers and the changes in the paper for each specific reviewer and annotate it with a note that mentions the corresponding reviewer point. 

We addressed all 13 points raised by the reviewers and conducted the necessary experiments, totaling 6486 CPU hours.




\section*{Reviewer 1}
\label{sec:reviewer1}

W1. The meta-learning method may be hard to support large input space and the change of environment. (D1-2)

D1. As shown in Table 8, it takes CAML about 12 days to train the meta-model to convergence based on the current meta-space with limited constraints. While the authors mentioned that CAML can support all constraints (Figure 3) simultaneously, it's quite important to estimate how much time it may take to generate sufficient training data from such a larger search space. Is the budget still endurable when there are a lot of constraints?

\answerVRone{\noindent\textbf{Answer:} We agree that the question of how our meta-training approach performs for an increasing number of constraints is interesting.

Therefore, we conducted an additional experiment comparing the meta-training for multiple constraints that we discuss in Section~\ref{sec:numberconstraintsmetatraining}. We ran one week of meta-training for different numbers of constraints and analyze the performance of the meta-model and its decline with increasing constraint space.
With increasing meta-training duration, the F1 score of the meta-model increases for all considered numbers of constraints. After one week, all constraint combinations reach an F1 score higher than $79\%$.
As expected, by adding additional constraints, the F1 score slightly decreases by up to 3\%, which is rather marginal considering the multiplied complexity of the resulting search space.  
This analysis can help to estimate how much time it may take to generate sufficient training data for larger search spaces.
}

D2. The authors mentioned how CAML supports the change of running environment, but the discussions seem too brief. They briefly introduce a solution that the users may use a benchmark to scale the performance from one environment to another. However, the scaling factor may differ from different feature engineering operations and ML algorithms. To obtain all factors, it requires additional budgets and efforts before the online phase begins. More discussions can be provided to show how to get those scaling factors and how the online phase adapts to new environments based on those scaling factors.

\answerVRone{\noindent\textbf{Answer:} We now expand the discussion on how to adapt the meta-model for a new hardware environment. In particular, we propose one simple calibration approach, which is independent of the underlying hardware. 
We evaluate this idea in Section~\ref{sec:hardwareajustmentexperiment}. The experiment shows that the proposed calibration approach successfully adjusts our meta-model to a new hardware environment.
}


D3. The main issue of the experiment is the absence of comparison under sufficient budget. It is expectable that CAML performs better than SOTA systems under limited budget as CAML switches off some time-consuming operations. However, it is also important to show whether CAML can achieve comparable results when the budget is sufficient (e.g., 30-60 min). This comparison shows whether CAML excessively switches off operations and algorithms or not.

\answerVRone{\noindent\textbf{Answer:} As suggested, we run CAML and all baselines for 30min and 60min and extend Table~\ref{tab:automlsys} accordingly.  
We discuss the new results in Section~\ref{subsec:experimentdiscussion}. As expected, relaxing the search time constraint diminishes the benefit of meta-learning as we do not need to optimize the search space. Please note that the premise of our paper is the application of AutoML in heavily constrained settings.  
}


D4. Similar to D3, to show how CAML works, it is suggested that the authors directly present the AutoML parameters when the search budget is 5s, 5min, and 60min on a specific task (Figure 5 shows the space on different datasets while Table 7 only shows the average change of selected algorithms). The changes between AutoML parameters under different constraints on the same task are interesting.

\answerVRone{\noindent\textbf{Answer:}
As suggested, we present the AutoML parameters when the search budget is 10s, 1min, and $\geq$~5min on the dataset ``numerai28.6'' in Table~\ref{tab:spacesonedata}.
Depending on the search time, \system{} modifies both the search space and the way it does training. For very short search time constraints and large datasets, it prefers incremental training to surface more models and pipelines. For higher search times, it considers more models and incorporates hold-out validation while avoiding incremental training because of the higher chance to overfit.
}


D5. Table 4 (the average frequency of algorithms chosen by CAML) is presented without further explanation. In Table 4, some algorithms have quite similar frequency under different constraints (e.g., MLP, HGB). Some even have larger frequency when the budget is quite low and high (e.g., LDA, SVC). More analysis should be provided to explain those results. In addition, the frequency using larger search budget can also be provided as mentioned in D3.

\answerVRone{\noindent\textbf{Answer:} As suggested, we extended the analysis in Section~\ref{sub:analysis} and, in addition, we provide the frequencies across classifiers for 30min and 60min in Table~\ref{tab:classifiers} as mentioned in D3. 

In particular, for some classifiers, such as MLP and HGB, the frequency stays similar across search time constraints. The reason is twofold: First, using incremental training, we can quickly yield working models for both classifier types that are competitive across search times. Second, \system{} identified that these classifier types work well for specific datasets which do not change across constraints. For instance, HGB was chosen for balanced datasets with fewer than 8 classes and more than 57 numeric features. MLP was chosen for skewed datasets with many categorical features.

Further analysis of classifiers, such as LDA and SVC, can be found in the paper. 
}



\section*{Reviewer 2}
\label{sec:reviewer2}

D1. The paper can benefit from explicitly mentioning how one adds a new constraint into the system. Does it require any effort at all? How does the user go about doing it?

\answerVRtwo{\noindent\textbf{Answer:} We clarified in the new Section~\ref{sec:extendconstraints}
 how to add a new constraint into the system:

The process differs depending on whether we are adding a search constraint or an application constraint.
For both cases, one has to define the user-defined function that describes the constraint. For ML application constraints, one has to implement the following template:

def constraint(pipeline, training\_time, X\_train, y\_train, X\_val, y\_val, threshold, constraint\_specific): True/False. This function takes the trained pipeline and its training time, the split data, the constraint threshold, and constraint-specific parameters, such as the sensitive attribute for fairness. The output of this function is whether the given ML pipeline passed the constraint or not.

After implementing the user-defined function, one has to add a new feature to the metadata representation and continue meta-training. To account for the new metadata feature, first one has to retrain the meta-model. With the retrained meta-model, one can continue alternating sampling including the new constraint.
Finally, one has to generate additional configurations that also cover the new constraint as described in Section~\ref{sec:mining}.

For search constraints, one has to additionally implement an initialize function that starts the measuring at the beginning of search and another function that checks whether the search constraint is still satisfied.
}

D2. Similarly, the evaluation section can benefit from experiments with several constraints at the same time, such as training time and equal opp., etc. It seems probable that, in practice, such compound constraints will likely come up.

\answerVRtwo{\noindent\textbf{Answer:} Thank you for this suggestion. As suggested, we added such experiments. We run experiments of all combinations of thresholds for 2\%, 4\%, 8\%, 16\%, and 32\% percentiles for both training time and equal opportunity (see Figure~\ref{figure:twoconstraints} - positive numbers mean that our dynamic approach outperforms the static one). Additionally, we conduct the same experiment for the combination of inference time and pipeline size (see Figure~\ref{figure:twoconstraints2}). 
%The computation of these experiments totals 917 CPU hours, which heavily weighs against our time and computation budget. 
We describe the new experiments and the results in Section~\ref{sec:twoconstrainteval}.

Generally, \emph{\system{} Dynamic} outperforms the static variant or achieves similar predictive performance in these experiments. Only for maximum restriction, such as 100\% equal opportunity or 4026B pipeline size, its performance was negligibly lower. Overall, the experiments show that \emph{\system{} Dynamic} works for multiple constraints and our meta-learning approach learns how these different constraints interact with each other. In 65\% of the cases, \system{} chooses AutoML configurations that consider two constraints simultaneously and were never chosen for the cases where we enforced only one of the constraints.
}

D3. It is not clear how in practice, one will come up with repositories of data sets and constraints to train the meta-model on. The paper can benefit from providing more background on that.

\answerVRtwo{\noindent\textbf{Answer:} We detailed in Section~\ref{sec:camlmain} how one can come up with repositories of data sets and constraints. 
For constraints, we provide training/inference time, pipeline size, and equal opportunity constraints. Scientists that want to extend this set can follow the conceptual steps now outlined in Section~\ref{sec:extendconstraints}. 

With regard to the repository of datasets, we acknowledge that the choice is crucial for the performance of meta-learning.
Meta-learning performs better if the user datasets are similar to the datasets that are present in the repository. In Section~\ref{sec:extendconstraints}, we explain two different ways to set up the repository. In short, the repository can either be targeted for a domain of tasks that are frequent inside an organization or one has to create the repository for multi-purpose tasks using a diversified set of datasets as we did in our benchmark using publicly available data. 
}

\section*{Reviewer 3}
\label{sec:reviewer3}

W1. I do not understand the necessity for constraining the search process to five minutes. Even matching the extremely large machine used in the evaluation, an equivalent AWS machine (r6g.12xlarge) costs \$2.419/hour, or \$0.20 for 5 minutes of compute. I am unsure of any organization, including extremely resource-constrained ones like universities, where \$0.20 is an excessive cost. 10 seconds would cost under 1 cent of compute. A standard setting is to run the model training overnight, which would be 8 hours of compute (minimum), costing \$19.352. 


As such, I believe the experiments should be redone with more realistic search settings, e.g., from coffee break (5 minutes) to overnight (8 hours).

\answerVRthree{\noindent\textbf{Answer:} As discussed for Point R1.D3, we conducted additional experiments for 30min and 60min as reported in Table~\ref{tab:automlsys}. The achieved average accuracy of the best AutoML system only changes at most 2\% between 30min and 60min. As all state-of-the-art AutoML systems converge at around 60min, we refrained from running experiments for higher time budgets. 
As expected, increasing the time budget reduces the necessity of search space optimization. 
%We note that on larger datasets, AutoML systems will potentially also need longer runtimes for convergences; but at the same time, each evaluation of an ML pipeline will take longer. Thus, we expect that in terms of the number of evaluations, the results will also translate to longer runtimes on larger datasets.
Generally, we would argue that the consideration of shorter search times is both important from an environmental point of view, as well as foundational research. Further, there are requirements for (near)real-time prediction as outlined in our introduction.}


W2. The paper is written entirely from the perspective of increasing the performance of AutoML. There is no discussion of how the results would play into data systems. As written, this paper is a much better fit for MLSys, OSDI/ATC, or NeurIPS/ICML. 

\answerVRthree{\noindent\textbf{Answer:} There has been extensive work on AutoML/ML systems in the data management community~\cite{DBLP:journals/pvldb/BoehmDEEMPRRSST16,shang2019democratizing,DBLP:conf/sigmod/ShahLKY021,boehm2019systemds,DBLP:conf/deem/HilprechtHR0B23}. We have added these references and contextualized our work in Section~\ref{sec:relatedwork}. Also the solution of this paper to specify constraints and let the AutoML system adapt its search space is on par with query optimization ideas in databases. Efficient AutoML is at the heart of many ML-based data preparation techniques. Optimizing it with regard to its resources will impact an end-to-end data science pipeline.}

D1. There are some bizarre statements in the text, such as "the search space is infinite" (page 2). While technically true, they do not really aid in understanding. As the authors are aware of, techniques such as Bayesian optimization can handle "infinite" search spaces.

\answerVRthree{\noindent\textbf{Answer:} As suggested, we reformulated the corresponding statements.}

D2. I am confused about the bolding in Table 1. Auto-sklearn2 opt has the same performance as CAML dynamic for 5 minutes (within the margin of error). Similarly, for Table 6 and 8 (too many to point out).

\answerVRthree{\noindent\textbf{Answer:} In Section~\ref{exp:setup}, we now clarified that in some cases the rounded average is very similar or the same, but one approach still passes the significance test to be better than the other approach. In these cases, we bold the results of the approach that passes the significance test.}


D3: Please report the CPU core types in the experimental evaluation.

\answerVRthree{\noindent\textbf{Answer:} Thank you for the suggestion. In Section~\ref{exp:setup}, we clarified that we use Intel(R) Xeon(R) Gold 6132 CPU @ 2.60GHz.}
